Rule-driven News Captioning

News captioning task aims to generate sentences by describing named entities or concrete events for an image with its news article. Existing methods have achieved remarkable results by relying on the large-scale pre-trained models, which primarily focus on the correlations between the input news content and the output predictions. However, the news captioning requires adhering to some fundamental rules of news reporting, such as accurately describing the individuals and actions associated with the event. In this paper, we propose the rule-driven news captioning method, which can generate image descriptions following designated rule signal. Specifically, we first design the news-aware semantic rule for the descriptions. This rule incorporates the primary action depicted in the image (e.g., "performing") and the roles played by named entities involved in the action (e.g., "Agent" and "Place"). Second, we inject this semantic rule into the large-scale pre-trained model, BART, with the prefix-tuning strategy, where multiple encoder layers are embedded with news-aware semantic rule. Finally, we can effectively guide BART to generate news sentences that comply with the designated rule. Extensive experiments on two widely used datasets (i.e., GoodNews and NYTimes800k) demonstrate the effectiveness of our method.

==> tab_statistics.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\begin{table}[!t]\small\renewcommand\arraystretch{1.7}
\centering
\captionsetup{justification=raggedright}
\caption{Name statistics in GoodNews and NYTimes800K.}
\label{tab:statistics}
\scalebox{1}
% \resizebox{\columnwidth}{}
{%
\begin{tabular}{lcc}
                            & GoodNews & NYTimes800K \\ \hline
Number of training captions & 421256   & 763217      \\
Number of people's names    & 284363   & 517117     \\
\multicolumn{1}{r}{\%}      & 67.50\%  & 67.75\%            \\ \hline
\end{tabular}%
}
\end{table}
